Pearl: A Review-driven Persona-Knowledge Grounded Conversational Recommendation Dataset

Conversational recommender system is an emerging area that has garnered an increasing interest in the community, especially with the advancements in large language models (LLMs) that enable diverse reasoning over conversational input. Despite the progress, the field has many aspects left to explore. The currently available public datasets for conversational recommendation lack specific user preferences and explanations for recommendations, hindering high-quality recommendations. To address such challenges, we present a novel conversational recommendation dataset named PEARL, synthesized with persona- and knowledge-augmented LLM simulators. We obtain detailed persona and knowledge from real-world reviews and construct a large-scale dataset with over 57k dialogues. Our experimental results demonstrate that utterances in PEARL include more specific user preferences, show expertise in the target domain, and provide recommendations more relevant to the dialogue context than those in prior datasets.

==> figure_latex/diversity.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/diversity_sample.png}
    \caption{Left: Statistics of inter-dialogue similarity, calculated with the TF-IDF vectors of dialogues. Right: Visualization of the TF-IDF vectors of dialogues by applying 2-dimensional Principal Component Analysis (PCA). We mark the regions that are specially correlated with the two datasets respectively.}
    \label{fig:diversity}
\end{figure}

==> figure_latex/human_eval.tex <==
% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{images/human_eval_sample.png}
%     \caption{Human evaluation results for dialogue quality. The scores (from 0 to 5) are averaged over all the samples rated by three annotators. $\kappa$ denotes Fleiss' Kappa, indicating fair or moderate inter-annotator agreement (0.2$<\kappa<$0.6).}
%     \label{fig:human_eval}
% \end{figure*}





\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/data_quality_inspired_result_temp.png}
    \caption{Results of head-to-head comparison human evaluation between conversations from \ourdata{} and those sampled from INSPIRED.}
    \label{fig:human_eval_inspired}
\end{figure}

==> figure_latex/item_diversity.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/item_diversity.png}
    \label{fig:item_diversity}
    \caption{item diversity.}
\end{figure}


==> figure_latex/scalability_figure.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/performance_per_size_sample.png}
    \caption{The effect on model performance by varying the number of dialogues, measured by R@1 and Dist-2.}
    \label{fig:scalability}
\end{figure}

==> tables/_main_table_rec.tex <==
\begin{table}
    \centering
    \small
    \begin{tabular}{ l c c c } 
        \toprule[1.0pt]
        Model & R@1  & R@10 & R@50   \\ 
        \toprule[1.0pt] 
        \multicolumn{4}{l}{\textbf{Evaluation on INSPIRED}} \\
        GPT-3.5  & 0.0389 & 0.1167 & 0.1984 \\
        \midrule
        \multicolumn{4}{l}{\textbf{Evaluation on \ourdata{}}} \\
        GPT-3.5  & 0.0071 & 0.0355 & 0.0709 \\
        \bottomrule[1.0pt]
    \end{tabular}
    \caption{Recommendation task performance of GPT-3.5 model on INSPIRED and \ourdata{}.}
    \label{tab:main_table_rec}
\end{table}





% \begin{table}
%     \centering
%     \small
%     \begin{tabular}{ l c c c c c } 
%         \toprule[1.0pt]
%         Model & Training data & R@1  & R@10 & R@50   \\ 
%         \toprule[1.0pt] 
%         \multicolumn{6}{l}{\textbf{Evaluation on INSPIRED}} \\
%         KBRD    & ReDial        & 0.05343 & 0.1755 & 0.3206 \\
%         KBRD    & \ourdata{}    & 0.007631 & 0.02290 & 0.09160 \\
%         BERT    & ReDial        & - & - & - \\
%         BERT    & \ourdata{}    & - & - & - \\
%         GPT-3.5-Turbo     &     -    & - & - & - \\
%         \midrule
%         \multicolumn{6}{l}{\textbf{Evaluation on \ourdata{}}} \\
%         KBRD    & ReDial        & - & - & - \\
%         KBRD    & \ourdata{}    & - & - & - \\
%         BERT    & ReDial        & - & - & - \\
%         BERT    & \ourdata{}    & - & - & - \\
%         GPT-3.5-Turbo     &     -    & - & - & - \\
%         \bottomrule[1.0pt]
%     \end{tabular}
%     \caption{Performance on INSPIRED and \ourdata{} when incorporating different types of training data.}
%     \label{tab:main_table}
% \end{table}





==> tables/case_study_poor.tex <==
{\renewcommand{\arraystretch}{1.35}
    \begin{table}[t] \begin{center}
    \small
    \setlength{\tabcolsep}{3pt}
    \begin{tabularx}{\linewidth}{X}
        \toprule
        \textbf{Recommender}: Hey there \\
        \textbf{Seeker}: Hi! I'm looking for recommendations on a great holiday movie, do you have any recommendations? \\
        \textbf{Recommender}: For sure! First, do you have certain preferences or aversions? Like are you into musicals? \\
        \textbf{Seeker}: I do not really like musicals. \\
        \textbf{Recommender}: Good to know... I would have recommended White Christmas, it's a classic and a bit of a tradition in our family, but there are so many to choose from! The old Tim Allen Santa Clause movie is super fun and so is Home Alone. \\
        \textbf{Seeker}: Is the Tim Allen Santa Clause movie funny? I would love to watch a funny movie. \\
        \textbf{Recommender}: Yes it is! It's a heart warming family comedy :) \\
        \textbf{Seeker}: I accept this recommendation and would love to watch it with my family! Thank you for your help. \\
        \textbf{Recommender}: You're very welcome! I hope you enjoy it! \\
        \textbf{Seeker}: If we finish this movie early, do you have children's Christmas movie to recommend? So far our favorite is Elf.
        \midrule
        \textbf{ReDial}: Yes, I love Elf! It's a great family movie! \\
        \textbf{Ours}: How about watching `The Lion King'? It's a classic animated film with a heartwarming story and memorable characters. It's perfect for family viewing and has a great message about family and friendship.
        \midrule
        \textbf{Ground-truth}: I would absolutely recommend Rise of the Guardians it's a kid's movie, but definitely funny so adults can enjoy too.
        \bottomrule
    \end{tabularx}
    \vspace{-3pt}
    \caption{
        Case study
    }
    \vspace{-10pt}
    \label{tab:example}
\end{center}\end{table}}



==> tables/human_eval_response.tex <==
{\renewcommand{\arraystretch}{1.3}
    \begin{table}[t!] \begin{center}
    \small
    \begin{adjustbox}{width=\columnwidth}
        \begin{tabular}{lcccc}
        % \begin{tabular}{@{}lcccc@{}}
            \toprule
            % Model                                   & Prosocial     & Engaged       & Respectful    & Coherent      & Overall   \\ 
            Model           & \rotatebox[origin=c]{0}{Naturalness}     & \rotatebox[origin=c]{0}{Relevance}       & \rotatebox[origin=c]{0}{Explainability}    & \rotatebox[origin=c]{0}{Overall}  \\ % & \rotatebox[origin=c]{45}{Overall}   \\ 
            \midrule                
            ReDial       & 33\%$^*$             & 47\%                 & 42\%$^*$             & 48\%            \\  % & 00\%                   \\
            \ourdata{}       & \textbf{67\%}$^*$    & \textbf{53\%}    & \textbf{58\%}$^*$    & \textbf{52\%}  \\  %  & \textbf{00\%}        \\
            \midrule                     % \\
            Reddit-ReDial     & 32\%$^*$            & 40\%$^*$             & 44\%             & 49\%            \\  % & 00\%                   \\
            \ourdata{}       & \textbf{68\%}$^*$    & \textbf{60\%}$^*$    & \textbf{55\%}    & \textbf{51\%}   \\  %  & \textbf{00\%}        \\
            \midrule        
            \midrule 
            Ground-truth  & 18\% $^*$             & 42\%$^*$             & 43\%$^*$             &37 \%$^*$            \\  % & 00\%                   \\
            \ourdata{}       & \textbf{82\%}$^*$    & \textbf{58\%}$^*$    & \textbf{57\%}$^*$    & \textbf{63\%}$^*$   \\  %  & \textbf{00\%}        \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
    \caption{Human evaluation results of responses from ChatGPT on DailyDialog when paired with DOCTOR vs. baseline models. ``w/o CS'' denotes direct response generation without commonsense knowledge. Win percentages with $^*$ indicate significance ($p < 0.05$). 
}
    \label{tab:rg_quality}
    \end{center}\end{table}
}


==> tables/main_table.tex <==


\begin{table*}
    \centering
    \small
    \begin{tabular}{ c c c c c c c c c} 
        \toprule[1.0pt]
          & \multicolumn{2}{c}{Training data} & \multicolumn{3}{c}{Recommendation}  & \multicolumn{3}{c}{Response generation} \\ 
          \cmidrule{2-3} \cmidrule{4-6} \cmidrule{7-9}
        Model & ReDial & \ourdata{} & R@1  & R@10 & R@50  & Dist-2 & Dist-3 & Dist-4  \\ 
        \toprule[1.0pt] 
        \multicolumn{9}{l}{\textbf{Evaluation on ReDial}} \\
        KGSF    & \cmark   &        & 1.96 & 1.09 & 0.33 & 1.08 & 0.68 &0.31   \\
        KGSF    &          & \cmark & 1.94 & 1.16 & 0.37 & 1.03 & 0.68 &0.38   \\
        KGSF    & \cmark   & \cmark & 1.95 & 0.98 & 0.29 & 0.97 & 0.42 &0.22   \\ \hdashline
        UniCRS  & \cmark   &        & 1.96 & 1.09 & 0.33 & 1.08 & 0.68 &0.31   \\
        UniCRS  &          & \cmark & 1.94 & 1.16 & 0.37 & 1.03 & 0.68 &0.38   \\
        UniCRS  & \cmark   & \cmark & 1.95 & 0.98 & 0.29 & 0.97 & 0.42 &0.22   \\
        \midrule
        \multicolumn{9}{l}{\textbf{Evaluation on INSPIRED}} \\
        KGSF    & \cmark   &        & 1.96 & 1.09 & 0.33 & 1.08 & 0.68 &0.31   \\
        KGSF    &          & \cmark & 1.94 & 1.16 & 0.37 & 1.03 & 0.68 &0.38   \\
        KGSF    & \cmark   & \cmark & 1.95 & 0.98 & 0.29 & 0.97 & 0.42 &0.22   \\ \hdashline
        UniCRS  & \cmark   &        & 1.96 & 1.09 & 0.33 & 1.08 & 0.68 &0.31   \\
        UniCRS  &          & \cmark & 1.94 & 1.16 & 0.37 & 1.03 & 0.68 &0.38   \\
        UniCRS  & \cmark   & \cmark & 1.95 & 0.98 & 0.29 & 0.97 & 0.42 &0.22   \\
        \bottomrule[1.0pt]
    \end{tabular}
    \caption{Performance on ReDial and INSPIRED when incorporating different types of training data.}
    \label{tab:main_table}
\end{table*}


==> tables/top_ngrams.tex <==
{\renewcommand{\arraystretch}{1.2}
    \begin{table}[t!] \begin{center}
    \begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{lcccccc}
        \toprule
        \multicolumn{7}{c}{Common keywords across all relations} \\
        \midrule  %
        \multicolumn{7}{c}{\makecell[c]{friendship, help, support, communication, family,\\car, happiness, school, success, work}} \\
        \bottomrule
        \toprule
                                    \multicolumn{7}{c}{Common keywords for each relation \footnotesize{(excluding the above)}} \\ 
        \midrule  %
        \makecell[c]{xAttr\\(18\%)}   & \multicolumn{6}{l}{\makecell[l]{kindness, anger, intelligent, responsibility, friend,\\trust, conversation, food, generosity, smart}}            \\
        \midrule
        \makecell[c]{xEffect\\(17\%)} & \multicolumn{6}{l}{\makecell[l]{gratitude, anger, upset, hard work, happy, money,\\friend, boss, party, kindness}}            \\
        \midrule
        \makecell[c]{xIntent\\(23\%)} & \multicolumn{6}{l}{\makecell[l]{independence, hard work, determination, money,\\relaxation, anger, kindness, store, understanding}}            \\
        \midrule
        \makecell[c]{xNeed\\(7\%)}    & \multicolumn{6}{l}{\makecell[l]{job, money, confidence, comfort, advice,\\interest, conversation, listening, store, park}}            \\
        \midrule
        \makecell[c]{xReact\\(25\%)}  & \multicolumn{6}{l}{\makecell[l]{frustration, anger, confidence, happy, pride, relief,\\disappointment, relaxation, anxiety, satisfaction}}            \\
        \midrule
        \makecell[c]{xWant\\(11\%)}   & \multicolumn{6}{l}{\makecell[l]{conversation, store, determination, apology, learning,\\doctor, job, friend, improvement, marriage}}            \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{
        Common topic keywords of the narratives (\ie conversation context) in \dataset.
        Numbers in parentheses denote the ratio of the relations in \dataset.
    }
    \vspace{-10pt}
    \label{tab:topic-keywords}
\end{center}\end{table}}


